On the Predictability of Talk Attendance at Academic Conferences

This paper focuses on the prediction of real-world talk attendances at academic conferences with respect to different influence factors. We study the predictability of talk attendances using real-world tracked face-to-face contacts. Furthermore, we investigate and discuss the predictive power of user interests extracted from the users' previous publications. We apply Hybrid Rooted PageRank, a state-of-the-art unsupervised machine learning method that combines information from different sources. Using this method, we analyze and discuss the predictive power of contact and interest networks separately and in combination. We find that contact and similarity networks achieve comparable results, and that combinations of different networks can only to a limited extend help to improve the prediction quality. For our experiments, we analyze the predictability of talk attendance at the ACM Conference on Hypertext and Hypermedia 2011 collected using the conference management system Conferator.

==> acknowledgements.tex <==
\section*{Acknowledgements}
This work has been supported by the VENUS research cluster at the interdisciplinary Research Center
  for Information System Design (ITeG) at Kassel University.
  
  We utilized active RFID technology which was developed within the SocioPatterns project, whose generous support we kindly acknowledge. 
Our particular thanks go the SocioPatterns team, especially to Ciro Cattuto, who enabled access to the SocioPatterns technology, 
and who supported us with valuable information concerning the setup of the RFID technology.


==> definition.tex <==
\section{Formal Model}\label{sec:model}









